Distilling Large Language Models for Biomedical Knowledge Extraction: A Case Study on Adverse Drug Events

Large language models (LLMs), such as GPT-4, have demonstrated remarkable capabilities across a wide range of tasks, including health applications. In this paper, we study how LLMs can be used to scale biomedical knowledge curation. We find that while LLMs already possess decent competency in structuring biomedical text, by distillation into a task-specific student model through self-supervised learning, substantial gains can be attained over out-of-box LLMs, with additional advantages such as cost, efficiency, and white-box model access. We conduct a case study on adverse drug event (ADE) extraction, which is an important area for improving care. On standard ADE extraction evaluation, a GPT-3.5 distilled PubMedBERT model attained comparable accuracy as supervised state-of-the-art models without using any labeled data. Despite being over 1,000 times smaller, the distilled model outperformed its teacher GPT-3.5 by over 6 absolute points in F1 and GPT-4 by over 5 absolute points. Ablation studies on distillation model choice (e.g., PubMedBERT vs BioGPT) and ADE extraction architecture shed light on best practice for biomedical knowledge extraction. Similar gains were attained by distillation for other standard biomedical knowledge extraction tasks such as gene-disease associations and protected health information, further illustrating the promise of this approach.

==> backup/1-intro.tex <==
\section{Introduction}

Adverse drug events (ADEs) pose a significant public health challenge, as they represent injuries resulting from medical interventions related to drug use, including medication errors, adverse drug reactions, allergic reactions, and overdoses~\citep{donaldson2000err}. In the United States, ADEs are prevalent in hospitals and are recognized as one of the leading causes of increased mortality, extended hospital stays, and elevated healthcare costs~\citep{classen1997adverse}. Identification and analysis of ADEs are essential for ensuring patient safety; however, manual review and information collection from narrative text data are typically labor-intensive and time-consuming~\citep{chen2020extracting}.

Automated systems for evidence-based pharmacovigilance can help address the challenges of manual ADE identification, particularly in pharmaceutical and healthcare companies~\citep{gurulingappa2012development}. However, constructing a gold standard corpus for ADE identification remains challenging due to the need for multiple specialized annotators with extensive biomedical backgrounds.

In this work, we address these challenges by exploring knowledge distillation from large language models (LLMs) and proposing a novel self-supervised end-to-end architecture for ADE extraction. 
Without using any human annotations, our method significantly outperforms GPT-4 and achieves comparable results to the fully supervised state of the art.
We also demonstrate the applicability of our method to other natural language processing tasks in the biomedical domain.

\subsection*{Generalizable Insights about Machine Learning in the Context of Healthcare}
\begin{itemize}
\item Knowledge distillation from LLMs and self supervision techniques boost the performance of information extraction tasks in the biomedical domain, which provides a general and reliable solution to various healthcare applications.

\item The proposed end-to-end architecture for ADE extraction underscores the importance of adapting machine learning models to the unique challenges and requirements of healthcare-related problems, increasing their relevance and impact in clinical settings.

\item The successful application of our approach to ADE extraction emphasizes the potential for transferring knowledge from LLMs to other natural language processing tasks in healthcare, contributing to a broader understanding of machine learning techniques in this domain.

\end{itemize}


\section{Related Work}

\subsection{End-to-end ADE Extraction}
A variety of approaches have been proposed in the field of Adverse Drug Event (ADE) extraction. Among these, SpERT \cite{eberts2019span} utilizes lightweight reasoning on BERT embeddings for joint entity and relation extraction, demonstrating the potential for combining these tasks. REBEL \cite{cabot2021rebel}, an autoregressive seq2seq model based on BART, simplifies relation extraction by representing triplets as text sequences and achieves state-of-the-art performance on multiple benchmarks. The table-sequence encoder model \cite{wang2020two} employs two distinct encoders to capture different information types during the learning process, showcasing significant improvements over existing single-encoder approaches.

\subsection{Knowledge Distillation via self Supervision}
Earlier large language models(LLM), such as GPT-3 \cite{ouyang2022training, agrawal2022large}, demonstrated potential but fell short of competitive results on biomedical NLP tasks \cite{gutierrez2022thinking, moradi2022gpt3}. However, the advent of GPT-3.5 and GPT-4 \cite{openai2023gpt4}, the latest generation of domain-agnostic large language models, has generated new opportunities for advancing medicine, health, and public understanding of the capabilities and limitations of these models \cite{lee2023ai}.

In this work, we concentrate on knowledge distillation of LLMs using self-supervision techniques \cite{agrawal2022large, smith2022language}. We leverage these LLMs as labelers in the biomedical domain, capitalizing on their powerful language understanding capabilities to generate high-quality labels effectively for various tasks. Our experiments highlight the advantages of this approach in enhancing performance on challenging biomedical NLP tasks, especially ADE extraction, emphasizing the potential of self-supervised distillation for harnessing the power of state-of-the-art LLMs in specialized domains.


==> backup/2-method.tex <==
\section{Methods}

% Tell us your techniques!  If your paper is develops a novel machine
% learning method or extension, then be sure to give the technical
% details---as you would for a machine learning publication---here and,
% as needed, in appendices.  If your paper is developing new methods
% and/or theory, this section might be several pages.

% If you are combining existing methods, feel free to cite other
% packages and papers and tell us how you put them together; that said,
% the work should stand alone for someone in that general machine
% learning area.  

\subsection{Task Definition}

In this study, we focus on the end-to-end ADE analysis: identifying mentions of adverse drug events within the given text, and classifying the relationships or causal links between the extracted ADE entities and drugs in the context. To validate our proposed method, we utilize the ADE corpus \citep{gurulingappa2012development}, a dataset systematically annotated for supporting the automatic extraction of drug-related adverse effects from medical reports.

The ADE corpus has undergone multiple rounds of double-annotation to ensure consistent and reliable annotations, providing mentions of ADEs as well as relations between drugs and ADEs. Since the dataset lacks an official train/dev/test split, we follow prior work and evaluate our method using 10-fold cross-validation. We report results in terms of lenient F1 score, as the primary metric in this study. This choice is motivated by the low inter-annotator agreement ratio reported in the dataset paper, and our observation of inconsistent mention boundaries of ADEs in the dataset, as detailed in \autoref{eval_method} and \autoref{tab:inconsistent-annotation}.


\subsection{A Unified Architecture for ADE Extraction and Causation Assignment}

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{ade model arch.png}
\caption{The proposed unified architecture for ADE extraction and causation assignment. The input sequence is processed to capture the final layer hidden state output for each drug entity. The hidden states are mean-pooled and concatenated to every hidden state output token, encoding drug information into each token. A linear layer is then applied for token classification using softmax, predicting ADE tokens while incorporating causation drug information. This architecture significantly reduces computational complexity from O(NM) to O(M), facilitating efficient and accurate large-scale ADE extraction and causation assignment.}
\label{fig:unified_arch}
\end{figure}

Traditional methods for Adverse Drug Event  extraction typically involve two separate subtasks: (1) identifying ADE mentions using Named Entity Recognition (NER), and (2) assigning causation to drugs through Relation Extraction (RE). In situations where multiple ADEs ($N$ mentions) and drugs ($M$ mentions) coexist in the same context, this approach necessitates $\mathcal{O}(NM)$ inferences, leading to a bottleneck for large-scale processing.

Recent studies \citep{santosh2021joint, cabot2021rebel} attempt to tackle this challenge by jointly extracting drug and ADE entities, even though \emph{drug extraction} has been largely addressed in prior work. In this paper, we propose a novel unified architecture that concentrates on the efficient and precise extraction of ADE entities and causation assignment. Our model introduces a drug-centric structure, designed to simultaneously handle ADE NER and RE in one pass.

As illustrated in \autoref{fig:unified_arch}, the input sequence undergoes processing to obtain the final layer hidden state output for each drug entity. Denote the input sequence as $x = {x_1, x_2, \ldots, x_T}$, where $x_i$ is the $i$-th token, and $T$ is the sequence length. The output of the final layer hidden state is represented as $H = {h_1, h_2, \ldots, h_T}$, where $h_i \in \mathbb{R}^d$ is the $d$-dimensional hidden state corresponding to the $i$-th token.

We then create a new input sequence for each drug entity. Given a set of drug entities $D = {d_1, d_2, \ldots, d_M}$, where $d_j$ is the $j$-th drug entity, for each drug, hidden states of drug entity are mean-pooled:

\begin{equation}
\bar{d}j = \frac{1}{T_j} \sum{i=1}^{T_j} d_{j,i}
\end{equation}

where $T_j$ is the number of tokens in the $j$-th drug entity, and $d_{j,i}$ is the $i$-th token of the $j$-th drug entity hidden state.

The resulting pooled token $\bar{d}_j$ is concatenated to every hidden state output token of the input sequence, effectively integrating drug information into each token:

\begin{equation}
\tilde{h}_{j,i} = \text{concat}(h_i, \bar{d}_j)
\end{equation}

where $\tilde{h}_{j,i} \in \mathbb{R}^{2d}$ is the concatenated hidden state for the $i$-th token in the new input sequence created for the $j$-th drug entity.

Subsequently, a linear layer is applied on top of the concatenated tokens for binary token classification using sigmoid. This process transforms the task into predicting ADE tokens while considering the causation drugs. The linear layer and sigmoid are defined as:

\begin{equation}
z_{j,i} = W \tilde{h}_{j,i} + b
\end{equation}

\begin{equation}
p_{j,i} = \sigma(z_{j,i}) = \frac{1}{1 + \exp(-z_{j,i})}
\end{equation}

where $W \in \mathbb{R}^{d'}$ and $b \in \mathbb{R}$ are learnable parameters of the linear layer, with $d' = 2d$ being the dimensionality of the concatenated hidden states, and $p_{j,i}$ represents the predicted probability of the $i$-th token in the new input sequence created for the $j$-th drug entity being an ADE mention.

The proposed architecture substantially simplifies the problem, converting the original two tasks (NER and RE) into a single, unified task. As a result, the computational requirement is dramatically reduced from O(NM) to O(M), enabling our end-to-end model to perform more efficiently and accurately in large-scale ADE extraction and causation assignment applications.

% \emph{Lack of technical details, such that the soundness of the
%   methods can be verified, is a major reason that otherwise
%   strong-looking papers are scored low/rejected.}


% \section{Cohort}

% \emph{This section is optional, and more theoretical work may not need
%   this section.  However, if you are using health data, then you need
%   to describe it carefully so that the clinicians can validate the
%   soundness of your choices.} 

% Describe the cohort.  Give us the details of any inclusion/exclusion
% criteria, what data were extracted, how features were processed,
% etc.  Recommended headings include:

% \subsection{Cohort Selection} 
% This includes choice of criteria and basic numbers, as well as any relevant
% information about the study design (such how cases and controls were
% identified, if appropriate), 

% \subsection{Data Extraction} 
% % This includes what raw information you extracted or collected, including any
% % assumptions and imputation that may have been used, and 


% \subsection{Feature Choices} 
% This includes how you might have converted the raw data into features that were
% used in your algorithm. 

% Cohort descriptions are just as important as methods details and code
% to replicate a study.  For more clinical application papers, each of
% the sections above might be several paragraphs because we really want
% to understand the setting.

% For the submission, please do \emph{not} include the name of the
% institutions for any private data sources.  However, in the
% camera-ready, you may include identifying information about the
% institution as well as should include any relevant IRB approval
% statements.




\subsection{Knowledge Distillation with LLM}

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{knowledge distillation_v4.png}
\caption{Figure 1: Self Supervision-Based Knowledge Distillation Framework for Training a Student Model with a LLM as Teacher: The schematic depicts the end-to-end process, beginning with the extraction of a curated corpus from the PubMed Database, followed by weak label generation using the LLM Teacher Model, and culminating with the optimization of the Student Model through training. This approach enables the Student Model to leverage the LLM's knowledge and performance while maintaining a more compact and efficient model size.}
\label{fig:distillation}
\end{figure}

We employ knowledge distillation (see Figure \ref{fig:distillation}) using GPT-3.5 as the teacher model.

\subsubsection{Data Curation and Preprocessing}

We adapt the methodology from Gurulingappa et al. \cite{gurulingappa2012development} to curate a corpus focused on drug-related adverse events. First, we perform a PubMed search with "drug therapy" and "adverse effects" as MeSH terms, limiting the language to English. This search yields approximately 50,000 PubMed abstracts related to drug-related adverse events. The query is as follows:
\begin{quote}
"adverse effects"[sh] AND (hasabstract[text] AND Case Reports[ptyp]) AND "drug therapy"[sh] AND English[lang] AND (Case Reports[ptyp])
\end{quote}

To efficiently recognize and normalize drug names in the abstracts, we compile a list of oncology drug names, synonyms, and abbreviations from the NCI Thesaurus. We construct a trie from this list for rapid search and identification within plain text. Next, we split each abstract into sentences, retaining only those containing identified drug names. This process results in a refined dataset suitable for knowledge distillation.

\subsubsection{Teacher and Student Models in Knowledge Distillation}

Our knowledge distillation process involves two models: the teacher model, which serves as the source of expertise, and the student model, which learns from the teacher model to achieve improved performance.

\textbf{Teacher Model:}
We employ GPT-3.5 as our teacher model. This advanced language model has demonstrated remarkable performance across various NLP tasks, showcasing its strong understanding and reasoning capabilities.

\textbf{Student Models:}
\begin{enumerate}
\item \textit{PubmedBERT}: PubmedBERT \cite{gu2021domain} and PubmedBERT Large \cite{tinn2021finetuning} are domain-specific language models pre-trained on PubMed abstracts and full-text articles from PubMed Central. These models have achieved state-of-the-art performance on numerous biomedical NLP tasks.
\item \textit{BioGPT}: BioGPT \cite{luo2022biogpt} is a domain-specific generative Transformer language model pre-trained on extensive biomedical literature. This model has demonstrated superior performance on six biomedical NLP tasks compared to previous models.
\end{enumerate}

\subsubsection{Knowledge Distillation Process}

We outline the knowledge distillation process, which includes generating input-output pairs, training the student models, and evaluating their performance using suitable prompts and post-processing techniques.

\textbf{Generate Input-Output Pairs:}
We split the collected corpus into sentences and input them to GPT-3.5. We then filter the responses to include only sentences with positive drug-ADE relations, and sample 40,000 sentences for student model training.

\textbf{Train the Student Models:}
We fine-tune the student models using the generated input-output pairs:
\begin{itemize}
\item \textit{PubmedBERT}: We fine-tune the entire model using the proposed architecture.
\item \textit{BioGPT}: We employ prefix soft tuning for the BioGPT model.
\end{itemize}

\textbf{Prompt Design:}
We experiment with zero-shot and few-shot settings, utilizing n-context learning or prompt-based learning. For the zero-shot setting, we provide a task description in the prompt and instruct the model to return 'none' if no ADE is found, which helps to reduce hallucination. For the few-shot setting, we use the same prompt and add five randomly sampled examples (Figure \ref{fig:ade_prompts}).

\textbf{Post-Processing:}
Although GPT-3.5 is initially used for span extraction, it struggles with span identification and tends to hallucinate. Instead, we ask for mentions and match the spans of mentions using regular expressions.

\textbf{Evaluation Metric:}
We employ the same evaluation metric for both supervised learning and the model-distilled self-supervision approaches, ensuring a fair comparison between the two methods. This metric accounts for the precision, recall, and F1-score, providing a comprehensive assessment of the models' performance in the drug-ADE relation prediction task.

\begin{figure}
\centering
\fbox{%
\parbox{\textwidth}{%
\textbf{Prompt}: Extract the adverse events each drug causes in the Message. If no ADE is found, return None.\

\textit{Example 1:}\\
Message: We postulate that the bolus of sulprostone resulted in possible coronary spasm that resulted in cardiac arrest.\\
Annotations: sulprostone: cardiac arrest$\vert$coronary spasm\\

\textit{Example 2:}\\
Message: In each of the three reported patients, alteration of eyelid appearance with deepening of the lid sulcus was evident as the result of topical bimatoprost therapy.\\
Annotations: bimatoprost: alteration of eyelid appearance$\vert$deepening of the lid sulcus\\

\textit{Example 3:}\\
Message: Immobilization, while Paget's bone disease was present, and perhaps enhanced activation of dihydrotachysterol by rifampicin, could have led to increased calcium - release into the circulation.\\
Annotations: dihydrotachysterol: increased calcium - release\\

\textit{Example 4:}\\
Message: In two patients clozapine was reinstated after risperidone was discontinued; serum triglyceride levels increased.\\
Annotations: clozapine: serum triglyceride levels increased\\

\textit{Example 5:}\\
Message: The cause of these previously unreported side effects of niacin therapy is uncertain but may be related to prostaglandin - mediated vasodilatation, hyperalgesia of sensory nerve receptors, and potentiation of inflammation in the gingiva with referral of pain to the teeth.\\
Annotations: niacin: hyperalgesia of sensory nerve receptors$\vert$pain to the teeth$\vert$potentiation of inflammation in the gingiva$\vert$prostaglandin - mediated vasodilatation
}
}
\caption{GPT-3.5 few-shot prompts for ADE extraction}
\label{fig:ade_prompts}
\end{figure}

==> backup/3-result.tex <==
% \subsection{Results on Synthetic Experiments}

% \emph{Depending on the claim you make in the paper, this section may
%   not be relevant.}

% Especially if you are developing a new method, you will want to
% demonstrate its properties on synthetic or semi-synthetic experiments.
% Include experiments that will help us understand the contribution of
% the work to machine learning and healthcare. 

\section{Results on Real Data}

\subsection{Evaluation Approach and Study Design} \label{eval_method}

To assess the efficacy of our proposed method, we first provide details on the evaluation approach and study design. The ADE dataset comprises 6,821 relations and 4,272 sentences. As no official train/dev/test split is provided, we divide the dataset into an 8:1:1 ratio for the following study.

We conduct an end-to-end evaluation wherein the correctness of an ADE is determined only when both entity extraction and its corresponding drug relation are accurate. However, due to the significantly low inter-annotator agreement ratio pertaining to the exact boundaries of ADE entities \cite{henry20202018}, we employ a relaxed matching approach that considers overlaps in the boundaries as sufficient. See Appendix \ref{tab:inconsistent-annotation} for examples.

\subsection{Supervised vs Distillation vs One- and Few-Shot Learning}

Our proposed supervised method achieved state-of-the-art performance, followed by the distilled PubMedBERT. The fine-tuned BioGPT performs slightly worse than GPT-3.5 in the few-shot setting, which aligns with its performance on end-to-end RE tasks as shown in \cite{luo2022biogpt}. We employ GPT-3.5 as the primary teacher model because, at the time of this study, GPT-4 had not yet been made available for large-scale inference calls.

As illustrated in Table 1 \ref{tab:res-distill}, our novel end-to-end architecture demonstrates promising performance in the extraction of ADE entities and identification of drug relationships. Furthermore, the knowledge distillation process involving GPT-3.5 as the teacher model and domain-specific models such as PubMedBERT and BioGPT as the student models enables efficient and accurate ADE extraction and causation assignment, contributing to the advancement of machine learning in healthcare.

During the knowledge distillation process, the student model learns from the teacher model by mimicking its output on a given set of examples. Although GPT-4 and GPT-3.5 are highly accurate, they still make precision or recall errors on certain examples. However, they also correctly annotate a large number of other examples. Given the massive amount of self-supervised annotations generated by GPT models, PubMedBERT is capable of identifying and rectifying such errors during its fine-tuning process.

Another reason behind this error denoising capability lies in the domain-specific nature of PubMedBERT. Being pretrained on a large corpus of biomedical literature, PubMedBERT already possesses substantial domain knowledge relevant to healthcare applications. This domain knowledge allows it to identify and correct the errors made by the more general GPT models.

% Present your numbers and be sure to compare proposed methods against appropriate baselines. 
% You should provide a summary of
% the results in the text, 
% as well as in tables (such as
% Table~\ref{tab:example}) and figures (such as
% Figure~\ref{fig:example}).  
% You may use subfigures/wrapfigures 
% so that figures don't have to span the whole page or multiple figures are side by side.



\begin{table}[t]
  \centering 
  \caption{Comparison of different methods on the ADE task. GPT 3.5 fewshot is used as teacher model in knowledge distillation process. The proposed task-specific model architecture (see Figure 1) is used in the supervised method. Lenient F1 is used as primary metric. }
  \begin{tabulary}{\textwidth}{l*{5}{>{\raggedright\arraybackslash}J}}
  \toprule
  
    \textbf{Method} & \textbf{Model} & \textbf{Corpus} & \textbf{Training labels}  &\textbf{Training size} & \textbf{Lenient F1}\\
    \midrule
    Supervised & PubMedBERT & ADE corpus & human annotation & 3,417 & 93.36 \\ 
    Distillation & PubMedBERT & PubMed abstracts & GPT 3.5 fewshot & 40,000 & 91.99 \\
    Supervised & BioGPT & ADE corpus & human annotation & 3,417 & 88.08 \\ 
    Few Shot & GPT 4 & ADE corpus & human annotation & 5 & 86.45 \\ 
    Few Shot & GPT 3.5 & ADE corpus & human annotation & 5 & 85.21 \\ 
    Zero Shot & GPT 4 & - & - & 0 & 84.92 \\ 
    Distillation & BioGPT & PubMed abstracts & GPT3.5 fewshot & 40,000 & 84.21 \\
    Zero Shot & GPT 3.5 & - & - & 0 & 78.22 \\ 
    \bottomrule
  \end{tabulary}
  \label{tab:res-distill} 

\end{table}





\subsection{self-supervised vs low resource supervised}
In this section, we compare the performance of self-supervised learning and low resource supervised learning on the ADE extraction task. Table \ref{tab:res-lowresource} presents the results for different methods, models, and training sizes. 

As shown in Table \ref{tab:res-lowresource}, the performance of the self-supervised method using PubMedBERT with GPT-3.5 fewshot (91.99 Lenient F1) is comparable to that of supervised learning with smaller training sizes (100-1,000 human-annotated examples). These results suggest that self-supervised learning can be an effective approach for ADE extraction, particularly when limited human-annotated examples are available.
\begin{table}[t]
  \centering 
  \caption{Comparison of distillation and low-resource supervised methods on the basis of Lenient F1 scores across various training sizes. As the training size decreases, the performance of the supervised model gradually degrades, with knowledge distillation offering a competitive alternative.}
    \begin{tabulary}{\textwidth}{l*{5}{>{\raggedright\arraybackslash}J}}
  \toprule
    \textbf{Method} & \textbf{Model} & \textbf{Corpus} & \textbf{Training labels}  &\textbf{Training size} & \textbf{Lenient F1}\\
    \midrule
    Supervised & PubMedBERT & ADE corpus & human annotation & 3,417 & 93.36 \\ 
    Supervised & PubMedBERT & ADE corpus & human annotation & 2,000 & 92.41 \\ 
    Supervised & PubMedBERT & ADE corpus & human annotation & 1,000 & 92.18 \\ 
    Distillation & PubMedBERT & PubMed abstract & GPT 3.5 fewshot & 40,000 & 91.99 \\
    Supervised & PubMedBERT & ADE corpus & human annotation & 500 & 91.51 \\ 
    Supervised & PubMedBERT & ADE corpus & human annotation & 100 & 89.33 \\ 
    \bottomrule
  \end{tabulary}
  \label{tab:res-lowresource} 
\end{table}

\subsection{supervised model architecture vs prior works}

To evaluate the performance of our supervised model architecture \ref{fig:unified_arch}, we conduct a comparative analysis with existing methods. Adhering to the methodology employed in prior works, we perform a 10-fold cross-validation. In this comparison, we utilize the end-to-end "strict" RE F1 score as our primary metric, which considers an ADE entity to be correct only when the span boundaries match precisely . This metric is selected as it has been consistently adopted in the referenced prior works for evaluation purposes.

\begin{table}[t]
  \centering 
  \caption{Comparison of the proposed eunified architecture with prior works in a supervised setting, evaluated using strict F1 scores as the primary metric. }
  \begin{tabular}{llllll}
  \toprule
    \textbf{Model} & \textbf{Strict f1}\\
    \midrule
    SpERT \cite{eberts2019span}& 79.24 \\ 
    Table-Sequence \cite{wang2020two} \cite{} & 80.01 \\ 
    SpERT.PL \cite{santosh2021joint} & 82.03 \\ 	
    REBEL \cite{cabot2021rebel} &82.2 \\
    Ours(PubMedBERT)& 84.27 \\ 
    Ours(PubMedBERT Large)& 84.53 \\ 

    \bottomrule
  \end{tabular}
  \label{tab:comp-prior} 
\end{table}
As shown in Table \ref{tab:comp-prior}, our proposed model using PubMedBERT outperforms prior works, achieving an F1 score of 84.27. Furthermore, when utilizing the larger version of PubMedBERT, the performance improves slightly to an F1 score of 84.53. These results indicate that our novel end-to-end architecture is highly effective in comparison to existing methods.

\subsection{LLM distillation on other clinical tasks}


we evaluate the impact of LLM distillation on other clinical tasks, as shown in Table \ref{tab:othertasks}. We provide a brief description of the clinical tasks mentioned:

\begin{itemize}
\item \textbf{GAD} - The Gene-Disease Association (GAD) \cite{becker2004genetic} task focuses on identifying associations between genes and diseases from biomedical literature. This task requires the extraction of gene and disease entities from text, as well as the determination of their relationships. The performance of models on this task is crucial for understanding genetic influences on diseases and advancing precision medicine.

\item \textbf{MEDNLI} - The Medical Natural Language Inference (MEDNLI) \cite{romanov2018lessons}task is based on the NLI task, which involves determining the relationship between a pair of sentences (entailment, contradiction, or neutral). In the context of MEDNLI, the sentences are derived from clinical text, making this task valuable for understanding complex relationships in medical documents.

\item \textbf{PHI(i2b2 2014)} - The Protected Health Information (PHI) task, specifically the i2b2 2014 shared task \cite{uzuner20142014}, aims at identifying and redacting personal identifiers in clinical text. The goal is to remove any information that could be used to trace back to individual patients, ensuring privacy and compliance with regulations such as the Health Insurance Portability and Accountability Act (HIPAA).
\end{itemize}

These clinical tasks present unique challenges and are essential for the development of machine learning models that can effectively process and understand biomedical and clinical text. By evaluating our proposed approach on these tasks, we can better understand its potential in various healthcare applications.

 In the GAD and PHI (i2b2 2014) tasks, model distillation using PubMedBERT performs better than the few-shot approach with GPT-3.5. However, for the MEDNLI task, the few-shot approach with GPT-3.5 slightly outperforms the model distillation with PubMedBERT. These results suggest that the effectiveness of knowledge distillation varies across different clinical tasks, and the choice of the best approach may depend on the specific requirements and characteristics of the task at hand.
\begin{table}[]
 \centering 
  \caption{LLM distillation on more clinical tasks}
\begin{tabular}{llll}
\textbf{task}  & \textbf{method}    & \textbf{model} & \textbf{f1} \\
\midrule
GAD            & Self-Supervised & PubMedBERT     & 56.42       \\
               & Few shot  & GPT 3.5        & 49.25       \\
MEDNLI         & Self-Supervised & PubMedBERT     & 80.24       \\
               & Few shot  & GPT 3.5        & 82.21       \\
PHI(i2b2 2014) & Self-Supervised & PubMedBERT     & 73.89       \\
               & Few shot  & GPT 3.5        & 64.20      \\
\bottomrule
\end{tabular}
  \label{tab:othertasks} 
\end{table}
% ACKNOWLEDGEMENTS ONLY GO IN THE CAMERA-READY, NOT THE SUBMISSION
% \acks{Many thanks to all collaborators and funders!}



==> backup/4-discussion.tex <==
\section{Discussion} 

% \emph{This is probably the most important section of your paper!  This
%   is where you tell us how your work advances our understanding of
%   machine learning and healthcare.}  Discuss both technical and
% clinical implications, as appropriate.
In this study, we presented a novel end-to-end architecture for ADE extraction, which combines entity recognition and relation extraction into a single framework. Our supervised model architecture, based on PubMedBERT, achieved state-of-the-art performance on the ADE dataset. We also demonstrated the effectiveness of knowledge distillation using GPT-3.5 as the teacher model and PubMedBERT and BioGPT as the student model for enhancing the performance of the model on the ADE extraction task. Furthermore, we showed that self-supervised learning with model distillation can achieve competitive results when compared to low-resource supervised learning.

Our evaluation of the proposed method on other clinical tasks, such as GAD, MEDNLI, and PHI (i2b2 2014), highlighted its potential for various healthcare applications. These results suggest that LLM distillation and domain-specific models, like PubMedBERT, can significantly contribute to the advancement of machine learning in healthcare.

% Future work could explore the incorporation of additional domain-specific knowledge sources or the development of novel architectures that further improve the performance of ADE extraction and other clinical tasks. Additionally, evaluating the proposed approach on a broader range of clinical tasks and datasets would help in understanding its generalizability and applicability in diverse healthcare scenarios.

\paragraph{Limitations}

% Explain when your approach may not apply, or things you could not
% check.  \emph{Discussing limitations is essential.  Both ACs and
%   reviewers have been advised to be skeptical of any work that does
%   not consider limitations.}
Despite the promising results, our study has several limitations:

Firstly, at the time of this work, the GPT-4 model had just been released. Due to time constraints, we did not conduct the distillation process using GPT-4 as the teacher model. In our few-shot setting, GPT-4 exhibited marginally better performance compared to GPT-3.5. Although we suspect that GPT-4 might be a better teacher, the expected gains are likely to be marginal.

Secondly, during the evaluation process, we assumed the presence of gold drug entities. This assumption is not held by several prior works that we compared our approach against. This difference in methodology might lead to a slight advantage in our setting, as our method relies on accurate drug entity identification to perform effectively.

Lastly, for knowledge distillation on other clinical tasks, we used the training corpus as input for the teacher model. However, given the relatively small size of these corpora, we have not been able to fully explore the true potential of distillation on these tasks. The limited data might restrict the effectiveness of the distillation process, and we acknowledge that there might be room for improvement with more extensive data and experimentation.

In summary, the limitations of our study include the use of GPT-3.5 instead of GPT-4 as the teacher model, the assumption of gold drug entities during evaluation, and the unexplored potential of distillation on other clinical tasks due to small training corpora. Future work could address these limitations by incorporating the latest language models, refining the evaluation process, and exploring the impact of larger training sets on knowledge distillation performance. 

\paragraph{Future Work}

To address the limitations and further enhance the performance of ADE extraction and other clinical tasks, several avenues for future research can be explored:

\begin{itemize}
\item \textit{Incorporating additional domain-specific knowledge sources}: Leveraging external domain-specific knowledge, such as ontologies and databases, could help improve model performance and address the issue of inconsistent annotations in the ADE dataset.
\item \textit{Expanding training corpus for other clinical tasks}: Increasing the training corpus for other clinical tasks using LLMs on unlabeled data could lead to improved performance in those tasks.
\item \textit{Evaluating on a broader range of clinical tasks and datasets}: Exploring the application of our proposed method on additional clinical tasks and datasets can provide further insights into the generalizability and adaptability of our approach in various healthcare contexts.
\item \textit{Investigating the use of GPT-4 in knowledge distillation}: Evaluating the potential benefits of incorporating GPT-4 in the knowledge distillation process could lead to further improvements in model performance across different clinical tasks.
\end{itemize}


==> backup_0422/1-intro.tex <==
\section{Introduction}

Adverse drug events (ADEs) pose a significant public health challenge, as they represent injuries resulting from medical interventions related to drug use, including medication errors, adverse drug reactions, allergic reactions, and overdoses~\citep{donaldson2000err}. In the United States, ADEs are prevalent in hospitals and are recognized as one of the leading causes of increased mortality, extended hospital stays, and elevated healthcare costs~\citep{classen1997adverse}. Identification and analysis of ADEs are essential for ensuring patient safety; however, manual review and information collection from narrative text data are typically labor-intensive and time-consuming~\citep{chen2020extracting}.

Automated systems for evidence-based pharmacovigilance can help address the challenges of manual ADE identification, particularly in pharmaceutical and healthcare companies~\citep{gurulingappa2012development}. However, constructing a gold standard corpus for ADE identification remains challenging due to the need for multiple specialized annotators with extensive biomedical backgrounds.

In this work, we address these challenges by exploring knowledge distillation from large language models (LLMs) and proposing a novel self-supervised end-to-end architecture for ADE extraction. 
Without using any human annotations, our method significantly outperforms GPT-4 and achieves comparable results to the fully supervised state of the art.
We also demonstrate the applicability of our method to other natural language processing tasks in the biomedical domain.

\subsection*{Generalizable Insights about Machine Learning in the Context of Healthcare}
\begin{itemize}
\item Knowledge distillation from LLMs and self supervision techniques boost the performance of information extraction tasks in the biomedical domain, which provides a general and reliable solution to various healthcare applications.

\item The proposed end-to-end architecture for ADE extraction underscores the importance of adapting machine learning models to the unique challenges and requirements of healthcare-related problems, increasing their relevance and impact in clinical settings.

\item The successful application of our approach to ADE extraction emphasizes the potential for transferring knowledge from LLMs to other natural language processing tasks in healthcare, contributing to a broader understanding of machine learning techniques in this domain.

\end{itemize}


\section{Related Work}

\subsection{End-to-end ADE Extraction}
A variety of approaches have been proposed in the field of Adverse Drug Event (ADE) extraction. Among these, SpERT \cite{eberts2019span} utilizes lightweight reasoning on BERT embeddings for joint entity and relation extraction, demonstrating the potential for combining these tasks. REBEL \cite{cabot2021rebel}, an autoregressive seq2seq model based on BART, simplifies relation extraction by representing triplets as text sequences and achieves state-of-the-art performance on multiple benchmarks. The table-sequence encoder model \cite{wang2020two} employs two distinct encoders to capture different information types during the learning process, showcasing significant improvements over existing single-encoder approaches.

\subsection{Knowledge Distillation via self Supervision}
Earlier large language models(LLM), such as GPT-3 \cite{ouyang2022training, agrawal2022large}, demonstrated potential but fell short of competitive results on biomedical NLP tasks \cite{gutierrez2022thinking, moradi2022gpt3}. However, the advent of GPT-3.5 and GPT-4 \cite{openai2023gpt4}, the latest generation of domain-agnostic large language models, has generated new opportunities for advancing medicine, health, and public understanding of the capabilities and limitations of these models \cite{lee2023ai}.

In this work, we concentrate on knowledge distillation of LLMs using self-supervision techniques \cite{agrawal2022large, smith2022language}. We leverage these LLMs as labelers in the biomedical domain, capitalizing on their powerful language understanding capabilities to generate high-quality labels effectively for various tasks. Our experiments highlight the advantages of this approach in enhancing performance on challenging biomedical NLP tasks, especially ADE extraction, emphasizing the potential of self-supervised distillation for harnessing the power of state-of-the-art LLMs in specialized domains.


==> backup_0422/2-method.tex <==
\section{Methods}

% Tell us your techniques!  If your paper is develops a novel machine
% learning method or extension, then be sure to give the technical
% details---as you would for a machine learning publication---here and,
% as needed, in appendices.  If your paper is developing new methods
% and/or theory, this section might be several pages.

% If you are combining existing methods, feel free to cite other
% packages and papers and tell us how you put them together; that said,
% the work should stand alone for someone in that general machine
% learning area.  

\subsection{Task Definition}

In this study, we focus on the end-to-end ADE analysis: identifying mentions of adverse drug events within the given text, and classifying the relationships or causal links between the extracted ADE entities and drugs in the context. To validate our proposed method, we utilize the ADE corpus \citep{gurulingappa2012development}, a dataset systematically annotated for supporting the automatic extraction of drug-related adverse effects from medical reports.

The ADE corpus has undergone multiple rounds of double-annotation to ensure consistent and reliable annotations, providing mentions of ADEs as well as relations between drugs and ADEs. Since the dataset lacks an official train/dev/test split, we follow prior work and evaluate our method using 10-fold cross-validation. We report results in terms of lenient F1 score, as the primary metric in this study. This choice is motivated by the low inter-annotator agreement ratio reported in the dataset paper, and our observation of inconsistent mention boundaries of ADEs in the dataset, as detailed in \autoref{eval_method} and \autoref{tab:inconsistent-annotation}.


\subsection{A Unified Architecture for ADE Extraction and Causation Assignment}

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{ade model arch.png}
\caption{The proposed unified architecture for ADE extraction and causation assignment. The input sequence is processed to capture the final layer hidden state output for each drug entity. The hidden states are mean-pooled and concatenated to every hidden state output token, encoding drug information into each token. A linear layer is then applied for token classification using softmax, predicting ADE tokens while incorporating causation drug information. This architecture significantly reduces computational complexity from O(NM) to O(M), facilitating efficient and accurate large-scale ADE extraction and causation assignment.}
\label{fig:unified_arch}
\end{figure}

Traditional methods for Adverse Drug Event  extraction typically involve two separate subtasks: (1) identifying ADE mentions using Named Entity Recognition (NER), and (2) assigning causation to drugs through Relation Extraction (RE). In situations where multiple ADEs ($N$ mentions) and drugs ($M$ mentions) coexist in the same context, this approach necessitates $\mathcal{O}(NM)$ inferences, leading to a bottleneck for large-scale processing.

Recent studies \citep{santosh2021joint, cabot2021rebel} attempt to tackle this challenge by jointly extracting drug and ADE entities, even though \emph{drug extraction} has been largely addressed in prior work. In this paper, we propose a novel unified architecture that concentrates on the efficient and precise extraction of ADE entities and causation assignment. Our model introduces a drug-centric structure, designed to simultaneously handle ADE NER and RE in one pass.

As illustrated in \autoref{fig:unified_arch}, the input sequence undergoes processing to obtain the final layer hidden state output for each drug entity. Denote the input sequence as $x = {x_1, x_2, \ldots, x_T}$, where $x_i$ is the $i$-th token, and $T$ is the sequence length. The output of the final layer hidden state is represented as $H = {h_1, h_2, \ldots, h_T}$, where $h_i \in \mathbb{R}^d$ is the $d$-dimensional hidden state corresponding to the $i$-th token.

We then create a new input sequence for each drug entity. Given a set of drug entities $D = {d_1, d_2, \ldots, d_M}$, where $d_j$ is the $j$-th drug entity, for each drug, hidden states of drug entity are mean-pooled:

\begin{equation}
\bar{d}j = \frac{1}{T_j} \sum{i=1}^{T_j} d_{j,i}
\end{equation}

where $T_j$ is the number of tokens in the $j$-th drug entity, and $d_{j,i}$ is the $i$-th token of the $j$-th drug entity hidden state.

The resulting pooled token $\bar{d}_j$ is concatenated to every hidden state output token of the input sequence, effectively integrating drug information into each token:

\begin{equation}
\tilde{h}_{j,i} = \text{concat}(h_i, \bar{d}_j)
\end{equation}

where $\tilde{h}_{j,i} \in \mathbb{R}^{2d}$ is the concatenated hidden state for the $i$-th token in the new input sequence created for the $j$-th drug entity.

Subsequently, a linear layer is applied on top of the concatenated tokens for binary token classification using sigmoid. This process transforms the task into predicting ADE tokens while considering the causation drugs. The linear layer and sigmoid are defined as:

\begin{equation}
z_{j,i} = W \tilde{h}_{j,i} + b
\end{equation}

\begin{equation}
p_{j,i} = \sigma(z_{j,i}) = \frac{1}{1 + \exp(-z_{j,i})}
\end{equation}

where $W \in \mathbb{R}^{d'}$ and $b \in \mathbb{R}$ are learnable parameters of the linear layer, with $d' = 2d$ being the dimensionality of the concatenated hidden states, and $p_{j,i}$ represents the predicted probability of the $i$-th token in the new input sequence created for the $j$-th drug entity being an ADE mention.

The proposed architecture substantially simplifies the problem, converting the original two tasks (NER and RE) into a single, unified task. As a result, the computational requirement is dramatically reduced from O(NM) to O(M), enabling our end-to-end model to perform more efficiently and accurately in large-scale ADE extraction and causation assignment applications.

% \emph{Lack of technical details, such that the soundness of the
%   methods can be verified, is a major reason that otherwise
%   strong-looking papers are scored low/rejected.}


% \section{Cohort}

% \emph{This section is optional, and more theoretical work may not need
%   this section.  However, if you are using health data, then you need
%   to describe it carefully so that the clinicians can validate the
%   soundness of your choices.} 

% Describe the cohort.  Give us the details of any inclusion/exclusion
% criteria, what data were extracted, how features were processed,
% etc.  Recommended headings include:

% \subsection{Cohort Selection} 
% This includes choice of criteria and basic numbers, as well as any relevant
% information about the study design (such how cases and controls were
% identified, if appropriate), 

% \subsection{Data Extraction} 
% % This includes what raw information you extracted or collected, including any
% % assumptions and imputation that may have been used, and 


% \subsection{Feature Choices} 
% This includes how you might have converted the raw data into features that were
% used in your algorithm. 

% Cohort descriptions are just as important as methods details and code
% to replicate a study.  For more clinical application papers, each of
% the sections above might be several paragraphs because we really want
% to understand the setting.

% For the submission, please do \emph{not} include the name of the
% institutions for any private data sources.  However, in the
% camera-ready, you may include identifying information about the
% institution as well as should include any relevant IRB approval
% statements.




\subsection{Knowledge Distillation with LLM}

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{knowledge distillation_v4.png}
\caption{Figure 1: Self Supervision-Based Knowledge Distillation Framework for Training a Student Model with a LLM as Teacher: The schematic depicts the end-to-end process, beginning with the extraction of a curated corpus from the PubMed Database, followed by weak label generation using the LLM Teacher Model, and culminating with the optimization of the Student Model through training. This approach enables the Student Model to leverage the LLM's knowledge and performance while maintaining a more compact and efficient model size.}
\label{fig:distillation}
\end{figure}

We employ knowledge distillation (see Figure \ref{fig:distillation}) using GPT-3.5 as the teacher model.

\subsubsection{Data Curation and Preprocessing}

We adapt the methodology from Gurulingappa et al. \cite{gurulingappa2012development} to curate a corpus focused on drug-related adverse events. First, we perform a PubMed search with "drug therapy" and "adverse effects" as MeSH terms, limiting the language to English. This search yields approximately 50,000 PubMed abstracts related to drug-related adverse events. The query is as follows:
\begin{quote}
"adverse effects"[sh] AND (hasabstract[text] AND Case Reports[ptyp]) AND "drug therapy"[sh] AND English[lang] AND (Case Reports[ptyp])
\end{quote}

To efficiently recognize and normalize drug names in the abstracts, we compile a list of oncology drug names, synonyms, and abbreviations from the NCI Thesaurus. We construct a trie from this list for rapid search and identification within plain text. Next, we split each abstract into sentences, retaining only those containing identified drug names. This process results in a refined dataset suitable for knowledge distillation.

\subsubsection{Teacher and Student Models in Knowledge Distillation}

Our knowledge distillation process involves two models: the teacher model, which serves as the source of expertise, and the student model, which learns from the teacher model to achieve improved performance.

\textbf{Teacher Model:}
We employ GPT-3.5 as our teacher model. This advanced language model has demonstrated remarkable performance across various NLP tasks, showcasing its strong understanding and reasoning capabilities.

\textbf{Student Models:}
\begin{enumerate}
\item \textit{PubmedBERT}: PubmedBERT \cite{gu2021domain} and PubmedBERT Large \cite{tinn2021finetuning} are domain-specific language models pre-trained on PubMed abstracts and full-text articles from PubMed Central. These models have achieved state-of-the-art performance on numerous biomedical NLP tasks.
\item \textit{BioGPT}: BioGPT \cite{luo2022biogpt} is a domain-specific generative Transformer language model pre-trained on extensive biomedical literature. This model has demonstrated superior performance on six biomedical NLP tasks compared to previous models.
\end{enumerate}

\subsubsection{Knowledge Distillation Process}

We outline the knowledge distillation process, which includes generating input-output pairs, training the student models, and evaluating their performance using suitable prompts and post-processing techniques.

\textbf{Generate Input-Output Pairs:}
We split the collected corpus into sentences and input them to GPT-3.5. We then filter the responses to include only sentences with positive drug-ADE relations, and sample 40,000 sentences for student model training.

\textbf{Train the Student Models:}
We fine-tune the student models using the generated input-output pairs:
\begin{itemize}
\item \textit{PubmedBERT}: We fine-tune the entire model using the proposed architecture.
\item \textit{BioGPT}: We employ prefix soft tuning for the BioGPT model.
\end{itemize}

\textbf{Prompt Design:}
We experiment with zero-shot and few-shot settings, utilizing n-context learning or prompt-based learning. For the zero-shot setting, we provide a task description in the prompt and instruct the model to return 'none' if no ADE is found, which helps to reduce hallucination. For the few-shot setting, we use the same prompt and add five randomly sampled examples (Figure \ref{fig:ade_prompts}).

\textbf{Post-Processing:}
Although GPT-3.5 is initially used for span extraction, it struggles with span identification and tends to hallucinate. Instead, we ask for mentions and match the spans of mentions using regular expressions.

\textbf{Evaluation Metric:}
We employ the same evaluation metric for both supervised learning and the model-distilled self-supervision approaches, ensuring a fair comparison between the two methods. This metric accounts for the precision, recall, and F1-score, providing a comprehensive assessment of the models' performance in the drug-ADE relation prediction task.

\begin{figure}
\centering
\fbox{%
\parbox{\textwidth}{%
\textbf{Prompt}: Extract the adverse events each drug causes in the Message. If no ADE is found, return None.\

\textit{Example 1:}\\
Message: We postulate that the bolus of sulprostone resulted in possible coronary spasm that resulted in cardiac arrest.\\
Annotations: sulprostone: cardiac arrest$\vert$coronary spasm\\

\textit{Example 2:}\\
Message: In each of the three reported patients, alteration of eyelid appearance with deepening of the lid sulcus was evident as the result of topical bimatoprost therapy.\\
Annotations: bimatoprost: alteration of eyelid appearance$\vert$deepening of the lid sulcus\\

\textit{Example 3:}\\
Message: Immobilization, while Paget's bone disease was present, and perhaps enhanced activation of dihydrotachysterol by rifampicin, could have led to increased calcium - release into the circulation.\\
Annotations: dihydrotachysterol: increased calcium - release\\

\textit{Example 4:}\\
Message: In two patients clozapine was reinstated after risperidone was discontinued; serum triglyceride levels increased.\\
Annotations: clozapine: serum triglyceride levels increased\\

\textit{Example 5:}\\
Message: The cause of these previously unreported side effects of niacin therapy is uncertain but may be related to prostaglandin - mediated vasodilatation, hyperalgesia of sensory nerve receptors, and potentiation of inflammation in the gingiva with referral of pain to the teeth.\\
Annotations: niacin: hyperalgesia of sensory nerve receptors$\vert$pain to the teeth$\vert$potentiation of inflammation in the gingiva$\vert$prostaglandin - mediated vasodilatation
}
}
\caption{GPT-3.5 few-shot prompts for ADE extraction}
\label{fig:ade_prompts}
\end{figure}

==> backup_0422/3-result.tex <==
% \subsection{Results on Synthetic Experiments}

% \emph{Depending on the claim you make in the paper, this section may
%   not be relevant.}

% Especially if you are developing a new method, you will want to
% demonstrate its properties on synthetic or semi-synthetic experiments.
% Include experiments that will help us understand the contribution of
% the work to machine learning and healthcare. 

\section{Results on Real Data}

\subsection{Evaluation Approach and Study Design} \label{eval_method}

To assess the efficacy of our proposed method, we first provide details on the evaluation approach and study design. The ADE dataset comprises 6,821 relations and 4,272 sentences. As no official train/dev/test split is provided, we divide the dataset into an 8:1:1 ratio for the following study.

We conduct an end-to-end evaluation wherein the correctness of an ADE is determined only when both entity extraction and its corresponding drug relation are accurate. However, due to the significantly low inter-annotator agreement ratio pertaining to the exact boundaries of ADE entities \cite{henry20202018}, we employ a relaxed matching approach that considers overlaps in the boundaries as sufficient. See Appendix \ref{tab:inconsistent-annotation} for examples.

\subsection{Supervised vs Distillation vs One- and Few-Shot Learning}

Our proposed supervised method achieved state-of-the-art performance, followed by the distilled PubMedBERT. The fine-tuned BioGPT performs slightly worse than GPT-3.5 in the few-shot setting, which aligns with its performance on end-to-end RE tasks as shown in \cite{luo2022biogpt}. We employ GPT-3.5 as the primary teacher model because, at the time of this study, GPT-4 had not yet been made available for large-scale inference calls.

As illustrated in Table 1 \ref{tab:res-distill}, our novel end-to-end architecture demonstrates promising performance in the extraction of ADE entities and identification of drug relationships. Furthermore, the knowledge distillation process involving GPT-3.5 as the teacher model and domain-specific models such as PubMedBERT and BioGPT as the student models enables efficient and accurate ADE extraction and causation assignment, contributing to the advancement of machine learning in healthcare.

During the knowledge distillation process, the student model learns from the teacher model by mimicking its output on a given set of examples. Although GPT-4 and GPT-3.5 are highly accurate, they still make precision or recall errors on certain examples. However, they also correctly annotate a large number of other examples. Given the massive amount of self-supervised annotations generated by GPT models, PubMedBERT is capable of identifying and rectifying such errors during its fine-tuning process.

Another reason behind this error denoising capability lies in the domain-specific nature of PubMedBERT. Being pretrained on a large corpus of biomedical literature, PubMedBERT already possesses substantial domain knowledge relevant to healthcare applications. This domain knowledge allows it to identify and correct the errors made by the more general GPT models.

% Present your numbers and be sure to compare proposed methods against appropriate baselines. 
% You should provide a summary of
% the results in the text, 
% as well as in tables (such as
% Table~\ref{tab:example}) and figures (such as
% Figure~\ref{fig:example}).  
% You may use subfigures/wrapfigures 
% so that figures don't have to span the whole page or multiple figures are side by side.



\begin{table}[t]
  \centering 
  \caption{Comparison of different methods on the ADE task. GPT 3.5 fewshot is used as teacher model in knowledge distillation process. The proposed task-specific model architecture (see Figure 1) is used in the supervised method. Lenient F1 is used as primary metric. }
  \begin{tabulary}{\textwidth}{l*{5}{>{\raggedright\arraybackslash}J}}
  \toprule
  
    \textbf{Method} & \textbf{Model} & \textbf{Corpus} & \textbf{Training labels}  &\textbf{Training size} & \textbf{Lenient F1}\\
    \midrule
    Supervised & PubMedBERT & ADE corpus & human annotation & 3,417 & 93.36 \\ 
    Distillation & PubMedBERT & PubMed abstracts & GPT 3.5 fewshot & 40,000 & 91.99 \\
    Supervised & BioGPT & ADE corpus & human annotation & 3,417 & 88.08 \\ 
    Few Shot & GPT 4 & ADE corpus & human annotation & 5 & 86.45 \\ 
    Few Shot & GPT 3.5 & ADE corpus & human annotation & 5 & 85.21 \\ 
    Zero Shot & GPT 4 & - & - & 0 & 84.92 \\ 
    Distillation & BioGPT & PubMed abstracts & GPT3.5 fewshot & 40,000 & 84.21 \\
    Zero Shot & GPT 3.5 & - & - & 0 & 78.22 \\ 
    \bottomrule
  \end{tabulary}
  \label{tab:res-distill} 

\end{table}





\subsection{self-supervised vs low resource supervised}
In this section, we compare the performance of self-supervised learning and low resource supervised learning on the ADE extraction task. Table \ref{tab:res-lowresource} presents the results for different methods, models, and training sizes. 

As shown in Table \ref{tab:res-lowresource}, the performance of the self-supervised method using PubMedBERT with GPT-3.5 fewshot (91.99 Lenient F1) is comparable to that of supervised learning with smaller training sizes (100-1,000 human-annotated examples). These results suggest that self-supervised learning can be an effective approach for ADE extraction, particularly when limited human-annotated examples are available.
\begin{table}[t]
  \centering 
  \caption{Comparison of distillation and low-resource supervised methods on the basis of Lenient F1 scores across various training sizes. As the training size decreases, the performance of the supervised model gradually degrades, with knowledge distillation offering a competitive alternative.}
    \begin{tabulary}{\textwidth}{l*{5}{>{\raggedright\arraybackslash}J}}
  \toprule
    \textbf{Method} & \textbf{Model} & \textbf{Corpus} & \textbf{Training labels}  &\textbf{Training size} & \textbf{Lenient F1}\\
    \midrule
    Supervised & PubMedBERT & ADE corpus & human annotation & 3,417 & 93.36 \\ 
    Supervised & PubMedBERT & ADE corpus & human annotation & 2,000 & 92.41 \\ 
    Supervised & PubMedBERT & ADE corpus & human annotation & 1,000 & 92.18 \\ 
    Distillation & PubMedBERT & PubMed abstract & GPT 3.5 fewshot & 40,000 & 91.99 \\
    Supervised & PubMedBERT & ADE corpus & human annotation & 500 & 91.51 \\ 
    Supervised & PubMedBERT & ADE corpus & human annotation & 100 & 89.33 \\ 
    \bottomrule
  \end{tabulary}
  \label{tab:res-lowresource} 
\end{table}

\subsection{supervised model architecture vs prior works}

To evaluate the performance of our supervised model architecture \ref{fig:unified_arch}, we conduct a comparative analysis with existing methods. Adhering to the methodology employed in prior works, we perform a 10-fold cross-validation. In this comparison, we utilize the end-to-end "strict" RE F1 score as our primary metric, which considers an ADE entity to be correct only when the span boundaries match precisely . This metric is selected as it has been consistently adopted in the referenced prior works for evaluation purposes.

\begin{table}[t]
  \centering 
  \caption{Comparison of the proposed eunified architecture with prior works in a supervised setting, evaluated using strict F1 scores as the primary metric. }
  \begin{tabular}{llllll}
  \toprule
    \textbf{Model} & \textbf{Strict f1}\\
    \midrule
    SpERT \cite{eberts2019span}& 79.24 \\ 
    Table-Sequence \cite{wang2020two} \cite{} & 80.01 \\ 
    SpERT.PL \cite{santosh2021joint} & 82.03 \\ 	
    REBEL \cite{cabot2021rebel} &82.2 \\
    Ours(PubMedBERT)& 84.27 \\ 
    Ours(PubMedBERT Large)& 84.53 \\ 

    \bottomrule
  \end{tabular}
  \label{tab:comp-prior} 
\end{table}
As shown in Table \ref{tab:comp-prior}, our proposed model using PubMedBERT outperforms prior works, achieving an F1 score of 84.27. Furthermore, when utilizing the larger version of PubMedBERT, the performance improves slightly to an F1 score of 84.53. These results indicate that our novel end-to-end architecture is highly effective in comparison to existing methods.

\subsection{LLM distillation on other clinical tasks}


we evaluate the impact of LLM distillation on other clinical tasks, as shown in Table \ref{tab:othertasks}. We provide a brief description of the clinical tasks mentioned:

\begin{itemize}
\item \textbf{GAD} - The Gene-Disease Association (GAD) \cite{becker2004genetic} task focuses on identifying associations between genes and diseases from biomedical literature. This task requires the extraction of gene and disease entities from text, as well as the determination of their relationships. The performance of models on this task is crucial for understanding genetic influences on diseases and advancing precision medicine.

\item \textbf{MEDNLI} - The Medical Natural Language Inference (MEDNLI) \cite{romanov2018lessons}task is based on the NLI task, which involves determining the relationship between a pair of sentences (entailment, contradiction, or neutral). In the context of MEDNLI, the sentences are derived from clinical text, making this task valuable for understanding complex relationships in medical documents.

\item \textbf{PHI(i2b2 2014)} - The Protected Health Information (PHI) task, specifically the i2b2 2014 shared task \cite{uzuner20142014}, aims at identifying and redacting personal identifiers in clinical text. The goal is to remove any information that could be used to trace back to individual patients, ensuring privacy and compliance with regulations such as the Health Insurance Portability and Accountability Act (HIPAA).
\end{itemize}

These clinical tasks present unique challenges and are essential for the development of machine learning models that can effectively process and understand biomedical and clinical text. By evaluating our proposed approach on these tasks, we can better understand its potential in various healthcare applications.

 In the GAD and PHI (i2b2 2014) tasks, model distillation using PubMedBERT performs better than the few-shot approach with GPT-3.5. However, for the MEDNLI task, the few-shot approach with GPT-3.5 slightly outperforms the model distillation with PubMedBERT. These results suggest that the effectiveness of knowledge distillation varies across different clinical tasks, and the choice of the best approach may depend on the specific requirements and characteristics of the task at hand.
\begin{table}[]
 \centering 
  \caption{LLM distillation on more clinical tasks}
\begin{tabular}{llll}
\textbf{task}  & \textbf{method}    & \textbf{model} & \textbf{f1} \\
\midrule
GAD            & Self-Supervised & PubMedBERT     & 56.42       \\
               & Few shot  & GPT 3.5        & 49.25       \\
MEDNLI         & Self-Supervised & PubMedBERT     & 80.24       \\
               & Few shot  & GPT 3.5        & 82.21       \\
PHI(i2b2 2014) & Self-Supervised & PubMedBERT     & 73.89       \\
               & Few shot  & GPT 3.5        & 64.20      \\
\bottomrule
\end{tabular}
  \label{tab:othertasks} 
\end{table}
% ACKNOWLEDGEMENTS ONLY GO IN THE CAMERA-READY, NOT THE SUBMISSION
% \acks{Many thanks to all collaborators and funders!}



==> backup_0422/4-discussion.tex <==
\section{Discussion} 

% \emph{This is probably the most important section of your paper!  This
%   is where you tell us how your work advances our understanding of
%   machine learning and healthcare.}  Discuss both technical and
% clinical implications, as appropriate.
In this study, we presented a novel end-to-end architecture for ADE extraction, which combines entity recognition and relation extraction into a single framework. Our supervised model architecture, based on PubMedBERT, achieved state-of-the-art performance on the ADE dataset. We also demonstrated the effectiveness of knowledge distillation using GPT-3.5 as the teacher model and PubMedBERT and BioGPT as the student model for enhancing the performance of the model on the ADE extraction task. Furthermore, we showed that self-supervised learning with model distillation can achieve competitive results when compared to low-resource supervised learning.

Our evaluation of the proposed method on other clinical tasks, such as GAD, MEDNLI, and PHI (i2b2 2014), highlighted its potential for various healthcare applications. These results suggest that LLM distillation and domain-specific models, like PubMedBERT, can significantly contribute to the advancement of machine learning in healthcare.

% Future work could explore the incorporation of additional domain-specific knowledge sources or the development of novel architectures that further improve the performance of ADE extraction and other clinical tasks. Additionally, evaluating the proposed approach on a broader range of clinical tasks and datasets would help in understanding its generalizability and applicability in diverse healthcare scenarios.

\paragraph{Limitations}

% Explain when your approach may not apply, or things you could not
% check.  \emph{Discussing limitations is essential.  Both ACs and
%   reviewers have been advised to be skeptical of any work that does
%   not consider limitations.}
Despite the promising results, our study has several limitations:

Firstly, at the time of this work, the GPT-4 model had just been released. Due to time constraints, we did not conduct the distillation process using GPT-4 as the teacher model. In our few-shot setting, GPT-4 exhibited marginally better performance compared to GPT-3.5. Although we suspect that GPT-4 might be a better teacher, the expected gains are likely to be marginal.

Secondly, during the evaluation process, we assumed the presence of gold drug entities. This assumption is not held by several prior works that we compared our approach against. This difference in methodology might lead to a slight advantage in our setting, as our method relies on accurate drug entity identification to perform effectively.

Lastly, for knowledge distillation on other clinical tasks, we used the training corpus as input for the teacher model. However, given the relatively small size of these corpora, we have not been able to fully explore the true potential of distillation on these tasks. The limited data might restrict the effectiveness of the distillation process, and we acknowledge that there might be room for improvement with more extensive data and experimentation.

In summary, the limitations of our study include the use of GPT-3.5 instead of GPT-4 as the teacher model, the assumption of gold drug entities during evaluation, and the unexplored potential of distillation on other clinical tasks due to small training corpora. Future work could address these limitations by incorporating the latest language models, refining the evaluation process, and exploring the impact of larger training sets on knowledge distillation performance. 

\paragraph{Future Work}

To address the limitations and further enhance the performance of ADE extraction and other clinical tasks, several avenues for future research can be explored:

\begin{itemize}
\item \textit{Incorporating additional domain-specific knowledge sources}: Leveraging external domain-specific knowledge, such as ontologies and databases, could help improve model performance and address the issue of inconsistent annotations in the ADE dataset.
\item \textit{Expanding training corpus for other clinical tasks}: Increasing the training corpus for other clinical tasks using LLMs on unlabeled data could lead to improved performance in those tasks.
\item \textit{Evaluating on a broader range of clinical tasks and datasets}: Exploring the application of our proposed method on additional clinical tasks and datasets can provide further insights into the generalizability and adaptability of our approach in various healthcare contexts.
\item \textit{Investigating the use of GPT-4 in knowledge distillation}: Evaluating the potential benefits of incorporating GPT-4 in the knowledge distillation process could lead to further improvements in model performance across different clinical tasks.
\end{itemize}

